Form factors and the dilatation operator in $\mathcal{N}=4$ super Yang-Mills theory and its deformations

In the first part of this thesis, we study form factors of general gauge-invariant local composite operators in $\mathcal{N}=4$ super Yang-Mills theory at various loop orders and for various numbers of external legs. We show how to use on-shell methods for their calculation and in particular extract the dilatation operator from the result. We also investigate the properties of the corresponding remainder functions. Moreover, we extend on-shell diagrams, a Gra{\ss}mannian integral formulation and an integrability-based construction via R-operators to form factors, focussing on the chiral part of the stress-tensor supermultiplet as an example. In the second part, we study the $\beta$- and the $\gamma_i$-deformation, which were respectively shown to be the most general supersymmetric and non-supersymmetric field-theory deformations of $\mathcal{N}=4$ super Yang-Mills theory that are integrable at the level of the asymptotic Bethe ansatz. For these theories, a new kind of finite-size effect occurs, which we call prewrapping and which emerges from double-trace structures that are required in the deformed Lagrangians. While the $\beta$-deformation is conformal when the double-trace couplings are at their non-trivial IR fixed points, the $\gamma_i$-deformation has running double-trace couplings without fixed points, which break conformal invariance even in the planar theory. Nevertheless, the $\gamma_i$-deformation allows for highly non-trivial field-theoretic tests of integrability at arbitrarily high loop orders.

==> picturemacro.tex <==
\makeatletter

%% Form factor diagrams
% xkeyval definitions
\define@boolkey{FDff}{oneloop}[true]{}
\define@boolkey{FDff}{twoloop}[true]{}
% \define@boolkey{FDff}{black}[true]{}
% \define@boolkey{FDff}{blue}[true]{}
% \define@boolkey{FDff}{green}[true]{}
\define@boolkey{FDff}{reflected}[true]{}
\define@boolkey{FDff}{fancy}[true]{}
% \define@boolkey{FDff}{small}[true]{}
% \define@key{FDff}{loops}%
%  {\def\FDffloops{#1}}%
\define@key{FDff}{legs}%
 {\def\FDfflegs{#1}}%
\define@key{FDff}{scaled}%
 {\def\FDffscaled{#1}}%
\presetkeys{FDff}{%
% loops=0,%
scaled=1,
legs=2,%
reflected=false,%
fancy=false,%
oneloop=false,%
twoloop=false%
% red=false,%
% bottomleglabel=$\phantom{0}$%
}{}
% Makro / FeynMP definitions
\newcommand*\FDff[1][]{%
 \setkeys{FDff}{#1}%
% 
\setlength{\unitlength}{\FDffscaled mm}%
\settoheight{\eqoff}{$\times$}%
\setlength{\eqoff}{0.5\eqoff}%
\addtolength{\eqoff}{-8\unitlength}%
\raisebox{\eqoff}{%
\fmfframe(1,1)(1,1){%
\scalebox{1}{%
\fmfstraight%
\begin{fmfchar*}(25,14)%
\expandafter\fmfcmd{%
dash_len := 0.5; 
newinternal numeric loops,legs,scald;
legs:=\FDfflegs;
scald:=\FDffscaled;
% loops:=\FDffloops;
}%
% \begin{fmfshrink}{1}
% outgoing
\ifKV@FDff@reflected
\fmfright{vq}
\fmfleftn{vp}{\FDfflegs}
\else
\fmfleft{vq}
\fmfrightn{vp}{\FDfflegs}
\fi
% internal lines left
\fmf{dbl_plain,tension=legs}{vq,v1}
% internal lines right
\ifKV@FDff@fancy
\fmf{plain}{v1,vp1}
\begin{fmffor}{n}{2}{1}{\FDfflegs-2}
\fmf{phantom}{v1,vp[n]}
\end{fmffor}
\begin{fmffor}{n}{\FDfflegs-1}{1}{\FDfflegs}
\fmf{plain}{v1,vp[n]}
\end{fmffor}
\else
\begin{fmffor}{n}{1}{1}{\FDfflegs}
\fmf{plain}{v1,vp[n]}
\end{fmffor}
\fi
\fmffreeze
\fmfdraw
 % labels  
 %%% Workaround for MetaPost 1.504 bug 
 \fmfcmd{pair vertq, vertpone, vertptwo, vertone; vertone = vloc(__v1); vertq = vloc(__vq); vertpone = vloc(__vp1); vertptwo = vloc(__vp2);}
 % lines
%  \fmfi{plain}{(vertone){dir 60}..{dir -45}(verttwo+(-20/sqrt(2),20/sqrt(2)))}
%  \fmfi{plain}{(vertone){dir -60}..{dir 45}(verttwo+(-20/sqrt(2),-20/sqrt(2)))}
%  \fmfi{plain}{(vertpone){dir -170}..{dir -135}(verttwo+(20/sqrt(2),20/sqrt(2)))}
%  \fmfi{plain}{(vertptwo){dir 170}..{dir 135}(verttwo+(20/sqrt(2),-20/sqrt(2)))}
 % blobs
%  \fmfiv{label=$\cF^{(1)}_{\cO}$,l.d=0,l.a=0}{vertone}
 % labels external states
%  \ifKV@FDff@spacetime
%  \fmfiv{label=$\scriptstyle q$}{vertq}
%  \fmfiv{label=$\scriptstyle p_1$}{vertpone}
%  \fmfiv{label=$\scriptstyle p_2$}{vertptwo}
% \else\fi
%  \fmfiv{label=$\cdot$,l.d=20,l.a=-45}{vertone}
%  \fmfiv{label=$\cdot$,l.d=20,l.a=-60}{vertone}
%  \fmfiv{label=$\cdot$,l.d=20,l.a=-75}{vertone}
% 
% \ifKV@FDff@flavour
%  \fmfiv{label=$\scriptstyle K$}{verttwo+(26,14)}
%  \fmfiv{label=$\scriptstyle I$}{verttwo+(-16,14)}
%  \fmfiv{label=$\scriptstyle L$}{verttwo+(26,-14)}
%  \fmfiv{label=$\scriptstyle J$}{verttwo+(-16,-14)}
% \else\fi
% 
% BLOB
  \fmfiv{decor.shape=circle,decor.filled=60,decor.size=30*scald}{vertone}
\ifKV@FDff@fancy
  \fmfiv{decor.shape=circle,decor.filled=0,decor.size=30*scald,label=$\ncsusyF_n$,l.d=0}{vertone}
  \ifKV@FDff@reflected
  \fmfiv{label=$\cdot$,l.d=20*scald,l.a=180}{vertone}
  \fmfiv{label=$\cdot$,l.d=20*scald,l.a=190}{vertone}
  \fmfiv{label=$\cdot$,l.d=20*scald,l.a=200}{vertone}
  \else
  \fmfiv{label=$\cdot$,l.d=20*scald,l.a=0}{vertone}
  \fmfiv{label=$\cdot$,l.d=20*scald,l.a=-10}{vertone}
  \fmfiv{label=$\cdot$,l.d=20*scald,l.a=-20}{vertone}
  \fi
\else\fi  
\ifKV@FDff@oneloop
  \fmfiv{decor.shape=circle,decor.filled=0,decor.size=15*scald}{vertone}
\else\fi
\ifKV@FDff@twoloop
\fmfcmd{fill (fullcircle scaled (15*scald) xscaled 0.5 shifted (vertone+(6*scald,0))) withcolor white;
draw (fullcircle scaled (15*scald) xscaled 0.5 shifted (vertone+(6*scald,0))) withcolor black;}
\fmfcmd{fill (fullcircle scaled (15*scald) xscaled 0.5 shifted (vertone+(-6*scald,0))) withcolor white;
draw (fullcircle scaled (15*scald) xscaled 0.5 shifted (vertone+(-6*scald,0))) withcolor black;}
%   \fmfiv{decor.shape=circle,decor.filled=0,decor.size=11}{vertone+(7,0)}
%   \fmfiv{decor.shape=circle,decor.filled=0,decor.size=11}{vertone+(-7,0)}
 \else\fi
% \end{fmfshrink}
\end{fmfchar*}%
\fmfcurved
}}}%
}




%% in-line diagrams
% xkeyval definitions
\define@boolkey{FDinline}{cutlabels}[true]{}
\define@boolkey{FDinline}{bubble}[true]{}
\define@boolkey{FDinline}{bubblethree}[true]{}
\define@boolkey{FDinline}{bubbletwoone}[true]{}
\define@boolkey{FDinline}{bubbletwoonerev}[true]{}
\define@boolkey{FDinline}{triangle}[true]{}
\define@boolkey{FDinline}{triangletwoone}[true]{}
\define@boolkey{FDinline}{triangletwoonerev}[true]{}
\define@boolkey{FDinline}{trianglethreetop}[true]{}
\define@boolkey{FDinline}{trianglethreebot}[true]{}
\define@boolkey{FDinline}{box}[true]{}
\define@boolkey{FDinline}{rainbow}[true]{}
\define@boolkey{FDinline}{fliprainbow}[true]{}
\define@boolkey{FDinline}{rainbownonplanar}[true]{}
\define@boolkey{FDinline}{fliprainbownonplanar}[true]{}
\define@boolkey{FDinline}{wedgetop}[true]{}
\define@boolkey{FDinline}{wedgebottom}[true]{}
\define@boolkey{FDinline}{wedgestartop}[true]{}
\define@boolkey{FDinline}{wedgestarbottom}[true]{}
\define@boolkey{FDinline}{itwo}[true]{}
\define@boolkey{FDinline}{fishtop}[true]{}
\define@boolkey{FDinline}{fishbottom}[true]{}
\define@boolkey{FDinline}{fishtopback}[true]{}
\define@boolkey{FDinline}{fishbottomback}[true]{}
\define@boolkey{FDinline}{trianglebubblethree}[true]{}
\define@boolkey{FDinline}{bubbletrianglethree}[true]{}
\define@boolkey{FDinline}{trianglesubbubbletop}[true]{}
\define@boolkey{FDinline}{trianglesubbubblebottom}[true]{}
\define@boolkey{FDinline}{trianglefishtop}[true]{}
\define@boolkey{FDinline}{trianglefishbottom}[true]{}
\define@boolkey{FDinline}{trianglefishtopback}[true]{}
\define@boolkey{FDinline}{trianglefishbottomback}[true]{}
\define@boolkey{FDinline}{trianglebridgebubbletop}[true]{}
\define@boolkey{FDinline}{trianglebridgebubblebottom}[true]{}
\define@boolkey{FDinline}{bubblevertical}[true]{}
\define@boolkey{FDinline}{sunrise}[true]{}
\define@boolkey{FDinline}{sunrisethree}[true]{}
\define@boolkey{FDinline}{bubbletriangle}[true]{}
\define@boolkey{FDinline}{doubletrianglethree}[true]{}
\define@boolkey{FDinline}{doubletriangletwo}[true]{}
\define@boolkey{FDinline}{doublebubble}[true]{}
\define@boolkey{FDinline}{boxtriangle}[true]{}
\define@boolkey{FDinline}{trianglebox}[true]{}
\define@boolkey{FDinline}{boxbubble}[true]{}
\define@boolkey{FDinline}{bubblebox}[true]{}
\define@boolkey{FDinline}{shiftedtriangletriangle}[true]{}
\define@boolkey{FDinline}{triangleshiftedtriangle}[true]{}
\define@boolkey{FDinline}{shiftedtrianglebubble}[true]{}
\define@boolkey{FDinline}{bubbleshiftedtriangle}[true]{}
\define@boolkey{FDinline}{masstop}[true]{}
\define@boolkey{FDinline}{massbottom}[true]{}
\define@boolkey{FDinline}{twomomenta}[true]{}
\define@boolkey{FDinline}{dermomenta}[true]{}
\define@boolkey{FDinline}{momentum}[true]{}
\define@boolkey{FDinline}{momentumarrow}[true]{}
\define@boolkey{FDinline}{altmomentum}[true]{}
\define@boolkey{FDinline}{twolabels}[true]{}
\define@boolkey{FDinline}{threelabels}[true]{}
\define@boolkey{FDinline}{cut}[true]{}
\define@boolkey{FDinline}{big}[true]{}
\define@boolkey{FDinline}{botdoublecut}[true]{}
\define@boolkey{FDinline}{topdoublecut}[true]{}
\define@boolkey{FDinline}{doublecut}[true]{}
\define@boolkey{FDinline}{slashdoublecut}[true]{}
\define@boolkey{FDinline}{bslashdoublecut}[true]{}
\define@boolkey{FDinline}{triplecut}[true]{}
\define@boolkey{FDinline}{alttriplecut}[true]{}
\define@boolkey{FDinline}{quadruplecut}[true]{}
\define@boolkey{FDinline}{splitlabels}[true]{}
\define@key{FDinline}{labelone}%
{\def\FDinlinelabelone{#1}}%
\define@key{FDinline}{labeltwo}%
{\def\FDinlinelabeltwo{#1}}%
\define@key{FDinline}{labelthree}%
{\def\FDinlinelabelthree{#1}}%
\define@key{FDinline}{toplabel}%
{\def\FDinlinetoplabel{#1}}%
\presetkeys{FDinline}{%
cutlabels=false,%
big=false,%
bubble=false,%
bubblethree=false,%
bubbletwoone=false,%
bubbletwoonerev=false,%
triangle=false,%
trianglethreetop=false,%
trianglethreebot=false,%
triangletwoone=false,%
triangletwoonerev=false,%
triangleshiftedtriangle=false,%
shiftedtriangletriangle=false,%
bubbleshiftedtriangle=false,%
shiftedtrianglebubble=false,%
box=false,%
rainbow=false,%
fliprainbow=false,%
rainbownonplanar=false,%
fliprainbownonplanar=false,%
wedgetop=false,%
wedgebottom=false,%
wedgestartop=false,%
wedgestarbottom=false,%
itwo=false,%
fishtop=false,%
fishbottom=false,%
fishtopback=false,%
fishbottomback=false,%
trianglesubbubbletop=false,%
trianglesubbubblebottom=false,%
trianglebridgebubbletop=false,%
trianglebridgebubblebottom=false,%
trianglefishtop=false,%
trianglefishbottom=false,%
trianglefishtopback=false,%
trianglefishbottomback=false,%
bubblevertical=false,%
sunrise=false,%
sunrisethree=false,%
massbottom=false,%
masstop=false,%
bubbletriangle=false,%
bubbletrianglethree=false,%
trianglebubblethree=false,%
bubblebox=false,%
boxbubble=false,%
trianglebox=false,%
boxtriangle=false,%
doubletriangletwo=false,%
doubletrianglethree=false,%
doublebubble=false,%
twomomenta=false,%
momentum=false,%
dermomenta=false,%
momentumarrow=false,%
altmomentum=false,%
twolabels=false,%
threelabels=false,%
cut=false,%
botdoublecut=false,%
topdoublecut=false,%
doublecut=false,%
slashdoublecut=false,%
bslashdoublecut=false,%
triplecut=false,%
alttriplecut=false,%
quadruplecut=false,%
splitlabels=false,%
toplabel=$\phantom{0}$,%
labelone=\phantom{0},%
labeltwo=\phantom{0},%
labelthree=\phantom{0}%
}{}
% Makro / FeynMP definitions
%straight galeries
\fmfstraight
\newcommand*\FDinline[1][]{%
 \setkeys{FDinline}{#1}%
% 
% BIG
\ifKV@FDinline@big
\unitlength=1mm
\else
\unitlength=0.6mm
\fi
%%% Distances for labels
% TWO LABELS  
 \ifKV@FDinline@twolabels
 \ifKV@FDinline@splitlabels
\ensuremath{\phantom{{\scriptstyle \FDinlinelabelone}}}
 \else\fi
 \else\fi
% THREE LABELS  
 \ifKV@FDinline@threelabels
 \ifKV@FDinline@splitlabels
\ensuremath{\phantom{{\scriptstyle \FDinlinelabelthree}}}
 \else\fi
 \else\fi
%%% diagrams
\settoheight{\eqoff}{$\times$}%
\setlength{\eqoff}{0.5\eqoff}%
\addtolength{\eqoff}{-11\unitlength}%
\raisebox{\eqoff}{%
\fmfframe(2,3)(2,3){%
\scalebox{1}{%
\begin{fmfchar*}(30,16)%
\fmfcmd{%
dash_len := 1.5mm; 
}%
% \begin{fmfshrink}{0.5}
\fmfstraight
% cut
\ifKV@FDinline@cut
\fmftop{vtop}
\fmfbottom{vbot}
\fmf{dashes}{vtop,vbot}
\else\fi
% BOX
\ifKV@FDinline@box
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
\fmftop{vt}
\fmfbottom{vb}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0}{v1,v2}
\fmf{plain,right=0}{v1,v3}
% internal lines right
\fmf{plain,tension=0.8}{v2,vp1}
\fmf{plain,tension=0.8}{v3,vp3}
% top and bottom
% \fmf{phantom,tension=1.8}{v2,vt}
% \fmf{phantom,tension=1.8}{v3,vb}
% right corner
% double cut
\ifKV@FDinline@doublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2}
\fmf{phantom_smallcut,right=0,tension=0}{v1,v3}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,left=0,tension=0}{v1,v2}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=right,right=0,tension=0}{v1,v3}
\else\fi
\else\fi
% slash double cut
\ifKV@FDinline@slashdoublecut
\fmf{phantom_smallcut,left=0,tension=0}{v2,v4}
\fmf{phantom_smallcut,right=0,tension=0}{v1,v3}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=10,label.side=left,left=0,tension=0}{v2,v4}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=right,right=0,tension=0}{v1,v3}
\else\fi
\else\fi
% back slash double cut
\ifKV@FDinline@bslashdoublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2}
\fmf{phantom_smallcut,right=0,tension=0}{v3,v4}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,left=0,tension=0}{v1,v2}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=10,label.side=right,right=0,tension=0}{v3,v4}
\else\fi
\else\fi
\fmffreeze
\fmf{plain,left=0}{v2,v4}
\fmf{plain,right=0}{v3,v4}
\fmf{plain,tension=5}{v4,vp2}
\else\fi
% BUBBLE
\ifKV@FDinline@bubble
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,label=\FDinlinetoplabel}{v1,v2}
\fmf{plain,right=0.7}{v1,v2}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,right=0.7,label=$\scriptstyle l$,l.d=2.5}{v2,v1}
\else\fi
% internal lines right
\fmf{plain,tension=1.5}{v2,vp1}
\fmf{plain,tension=1.5}{v2,vp2}
% double cut
\ifKV@FDinline@doublecut
\fmf{phantom_smallcut,left=0.7,tension=0}{v1,v2}
\fmf{phantom_smallcut,right=0.7,tension=0}{v1,v2}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,left=0.7,tension=0}{v1,v2}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=right,right=0.7,tension=0}{v1,v2}
\else\fi
\else\fi
\else\fi
% BUBBLETHREE
\ifKV@FDinline@bubblethree
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,label=\FDinlinetoplabel}{v1,v2}
\fmf{plain,right=0.7}{v1,v2}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,right=0.7,label=$\scriptstyle l$,l.d=2.5}{v2,v1}
\else\fi
% double cut
\ifKV@FDinline@doublecut
\fmf{phantom_smallcut,left=0.7,tension=0}{v1,v2}
\fmf{phantom_smallcut,right=0.7,tension=0}{v1,v2}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,left=0.7,tension=0}{v1,v2}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=right,right=0.7,tension=0}{v1,v2}
\else\fi
\else\fi
% two momenta
\ifKV@FDinline@twomomenta
\fmf{electron,tension=0,right=0.7,label=$\scriptstyle l_1$}{v2,v1}
\fmf{electron,tension=0,left=0.7,label=$\scriptstyle l_2$}{v2,v1}
\else\fi
% internal lines right
\fmf{plain,tension=1.5}{v2,vp1}
\fmf{plain,tension=1.5}{v2,vp2}
\fmf{plain,tension=1.5}{v2,vp3}
\else\fi
% BUBBLETWOONE
\ifKV@FDinline@bubbletwoone
% outgoing
\fmfleft{vq,vp3}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=1.5}{vq,v1}
\fmf{plain,tension=1.5}{vp3,v1}
% internal lines middle
\fmf{plain,left=0.7,label=\FDinlinetoplabel}{v1,v2}
\fmf{plain,right=0.7}{v1,v2}
% internal lines right
\fmf{plain,tension=1.5}{v2,vp1}
\fmf{plain,tension=1.5}{v2,vp2}
\else\fi
% BUBBLETWOONEREV
\ifKV@FDinline@bubbletwoonerev
% outgoing
\fmfleft{vp3,vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=1.5}{vq,v1}
\fmf{plain,tension=1.5}{vp3,v1}
% internal lines middle
\fmf{plain,left=0.7,label=\FDinlinetoplabel}{v1,v2}
\fmf{plain,right=0.7}{v1,v2}
% internal lines right
\fmf{plain,tension=1.5}{v2,vp1}
\fmf{plain,tension=1.5}{v2,vp2}
\else\fi
% BUBBLE VERTICAL
\ifKV@FDinline@bubblevertical
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,tag=1,tension=0.5}{v1,v2}
\fmf{plain,left=0.7,tag=2,tension=0.5}{v2,v1}
% internal lines right
\fmf{plain,tension=2}{v2,vp1}
\fmf{plain,tension=2}{v2,vp2}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2)}
\fmfiset{p2}{vpath2(__v2,__v1)}
\fmfi{plain}{point length(p1)/2 of p1
-- point length(p2)/2 of p2}
\else\fi
% FISHTOP
\ifKV@FDinline@fishtop
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,tag=1,tension=0.5}{v1,v2}
\fmf{plain,left=0.7,tag=2,tension=0.5}{v2,v1}
% momentumarrow
\ifKV@FDinline@momentumarrow
\fmf{electron,tension=0,left=0.7}{v2,v1}
\else\fi
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0.7,label=$\scriptstyle l$,l.d=2.5}{v2,v1}
\else\fi
% internal lines right
\fmf{plain,tension=2}{v2,vp1}
\fmf{plain,tension=2}{v2,vp2}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2)}
\fmfiset{p2}{vpath2(__v2,__v1)}
\fmfi{plain}{(point length(p1)/2 of p1){dir -90}..{dir 180}(point length(p2) of p2)}
\fmffreeze
% triple cut
\ifKV@FDinline@triplecut
\fmfi{phantom_smallcut}{(point length(p1)/2 of p1){dir -90}..{dir 180}(point length(p2) of p2)}
\fmfi{phantom_smallcut}{subpath (0,0.5*length(p1)) of p1}
\fmfi{phantom_smallcut}{subpath (length(p2),0*length(p2)) of p2}
\else\fi
% cutlabels
\ifKV@FDinline@cutlabels
% \fmfi{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$}{(point length(p1)/2 of p1){dir -90}..{dir 180}(point length(p2) of p2)}
\fmfi{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$}{subpath (0,0.5*length(p1)) of p1}
\fmfi{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$}{subpath (length(p2),0*length(p2)) of p2}
 \fmfcmd{pair vert; vert = vloc(__v1);}
 % labels
 \fmfiv{label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.a=0,l.d=15}{vert}
\else\fi
\else\fi
% FISHBOTTOMBACK
\ifKV@FDinline@fishbottomback
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,tag=1,tension=0.5}{v1,v2}
\fmf{plain,left=0.7,tag=2,tension=0.5}{v2,v1}
% internal lines right
\fmf{plain,tension=2}{v2,vp1}
\fmf{plain,tension=2}{v2,vp2}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2)}
\fmfiset{p2}{vpath2(__v2,__v1)}
\fmfi{plain}{(point length(p2)/2 of p2){dir 90}..{dir 0}(point length(p1) of p1)}
\else\fi
% FISHTOPBACK
\ifKV@FDinline@fishtopback
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,tag=1,tension=0.5}{v1,v2}
\fmf{plain,left=0.7,tag=2,tension=0.5}{v2,v1}
% internal lines right
\fmf{plain,tension=2}{v2,vp1}
\fmf{plain,tension=2}{v2,vp2}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2)}
\fmfiset{p2}{vpath2(__v2,__v1)}
\fmfi{plain}{(point length(p1)/2 of p1){dir -90}..{dir 0}(point 0length(p2) of p2)}
\else\fi
% FISHBOTTOM
\ifKV@FDinline@fishbottom
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,tag=1,tension=0.5}{v1,v2}
\fmf{plain,left=0.7,tag=2,tension=0.5}{v2,v1}
% momentumarrow
\ifKV@FDinline@momentumarrow
\fmf{electron,tension=0,right=0.7}{v2,v1}
\else\fi
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,right=0.7,label=$\scriptstyle l$,l.d=2.5}{v2,v1}
\else\fi
% internal lines right
\fmf{plain,tension=2}{v2,vp1}
\fmf{plain,tension=2}{v2,vp2}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2)}
\fmfiset{p2}{vpath2(__v2,__v1)}
\fmfi{plain}{(point length(p2)/2 of p2){dir 90}..{dir 180}(point 0length(p1) of p1)}
% triple cut
\ifKV@FDinline@triplecut
\fmfi{phantom_smallcut}{(point length(p2)/2 of p2){dir 90}..{dir 180}(point 0length(p1) of p1)}
\fmfi{phantom_smallcut}{subpath (length(p2),0.5*length(p2)) of p2}
\fmfi{phantom_smallcut}{subpath (length(p1),0*length(p1)) of p1}
\else\fi
% cutlabels
\ifKV@FDinline@cutlabels
% \fmfi{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$}{(point length(p2)/2 of p2){dir 90}..{dir 180}(point 0length(p1) of p1)}
\fmfi{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$}{subpath (length(p2),0.5*length(p2)) of p2}
\fmfi{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$}{subpath (length(p1),0*length(p1)) of p1}
 \fmfcmd{pair vert; vert = vloc(__v1);}
 % labels
 \fmfiv{label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.a=0,l.d=15}{vert}
\else\fi
\else\fi
% SUNRISE
\ifKV@FDinline@sunrise
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,label=\FDinlinetoplabel,tension=0.5}{v1,v2}
\fmf{plain,right=0.7,tension=0.5}{v1,v2}
\fmf{plain,right=0,tension=0}{v1,v2}
% internal lines right
\fmf{plain,tension=1.5}{v2,vp1}
\fmf{plain,tension=1.5}{v2,vp2}
\fmffreeze
% triple cut
\ifKV@FDinline@triplecut
\fmf{phantom_smallcut,left=0.7,tension=0}{v1,v2}
\fmf{phantom_smallcut,right=0.7,tension=0}{v1,v2}
\fmf{phantom_smallcut,right=0,tension=0}{v1,v2}
\else\fi
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,left=0.7,tension=0}{v1,v2}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,right=0.7,tension=0}{v1,v2}
 \fmfcmd{pair vert; vert = vloc(__v1);}
 % labels
 \fmfiv{label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.a=-15,l.d=18}{vert}
% \fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,right=0,tension=0}{v1,v2}
\else\fi
\else\fi
% SUNRISETHREE
\ifKV@FDinline@sunrisethree
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,tension=0.5,label=\FDinlinetoplabel}{v1,v2}
\fmf{plain,right=0.7,tension=0.5}{v1,v2}
\fmf{plain,right=0,tension=0}{v1,v2}
% internal lines right
\fmf{plain,tension=1.5}{v2,vp1}
\fmf{plain,tension=1.5}{v2,vp2}
\fmf{plain,tension=1.5}{v2,vp3}
\else\fi
% DOUBLEBUBBLE
\ifKV@FDinline@doublebubble
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.7,label=\FDinlinetoplabel}{v1,v2}
\fmf{plain,right=0.7}{v1,v2}
% internal lines middle right
\fmf{plain,left=0.7,label=\FDinlinetoplabel}{v2,v3}
\fmf{plain,right=0.7}{v2,v3}
% internal lines right
\fmf{plain,tension=1.5}{v3,vp1}
\fmf{plain,tension=1.5}{v3,vp2}
\else\fi
% BUBBLETRIANGLE
\ifKV@FDinline@bubbletriangle
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,label=\FDinlinetoplabel}{v1,v2}
\fmf{plain,right=0.7}{v1,v2}
% internal lines middle
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v2,v2t}
\fmf{plain,right=0.0}{v2,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% internal lines right
\fmf{plain,tension=1.5}{v2t,vp1}
\fmf{plain,tension=1.5}{v2b,vp2}
\else\fi
% TRIANGLE
\ifKV@FDinline@triangle
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% internal lines right
\fmf{plain,tension=1.5}{v2t,vp1}
\fmf{plain,tension=1.5}{v2b,vp2}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,right=0,label=$\scriptstyle l$,l.d=2.5,label.side=right}{v2t,v1}
\else\fi
% double cut
\ifKV@FDinline@doublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2t}
\fmf{phantom_smallcut,right=0,tension=0}{v1,v2b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,left=0,tension=0}{v1,v2t}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=right,right=0,tension=0}{v1,v2b}
\else\fi
\else\fi
% triple cut
\ifKV@FDinline@triplecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2t}
\fmf{phantom_smallcut,right=0,tension=0}{v1,v2b}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v2b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,left=0,tension=0}{v1,v2t}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=right,right=0,tension=0}{v1,v2b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,l.d=8,label.side=left,right=0,tension=0}{v2t,v2b}
\else\fi
\else\fi
\else\fi
% TRIANGLEBRIDGEBUBBLETOP
\ifKV@FDinline@trianglebridgebubbletop
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
% internal lines right
\fmf{plain,tension=2}{v2t,vp1}
\fmf{plain,tension=2}{v2b,vp2}
\fmffreeze
% middle
\fmf{plain,tension=3}{vm,v2b}
\fmf{plain,tension=1,left=0.5}{vm,v2t}
\fmf{plain,tension=1,right=0.5}{vm,v2t}
\else\fi
% TRIANGLEBRIDGEBUBBLEBOTTOM
\ifKV@FDinline@trianglebridgebubblebottom
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
% internal lines right
\fmf{plain,tension=2}{v2t,vp1}
\fmf{plain,tension=2}{v2b,vp2}
\fmffreeze
% middle
\fmf{plain,tension=3}{vm,v2t}
\fmf{plain,tension=1,left=0.5}{vm,v2b}
\fmf{plain,tension=1,right=0.5}{vm,v2b}
\else\fi
% TRIANGLETWOONE
\ifKV@FDinline@triangletwoone
% outgoing
\fmfleft{vq,vp3}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=1.5}{vq,v1}
\fmf{plain,tension=1.5}{vp3,v1}
% internal lines middle
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% internal lines right
\fmf{plain,tension=1.5}{v2t,vp1}
\fmf{plain,tension=1.5}{v2b,vp2}
\else\fi
% TRIANGLETWOONEREV
\ifKV@FDinline@triangletwoonerev
% outgoing
\fmfleft{vp3,vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=1.5}{vq,v1}
\fmf{plain,tension=1.5}{vp3,v1}
% internal lines middle
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% internal lines right
\fmf{plain,tension=1.5}{v2t,vp1}
\fmf{plain,tension=1.5}{v2b,vp2}
\else\fi
% TRIANGLETHREETOP
\ifKV@FDinline@trianglethreetop
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% internal lines right
\fmf{plain,tension=1.5}{v2t,vp1}
\fmf{plain,tension=0}{v2t,vp2}
\fmf{plain,tension=1.5}{v2b,vp3}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,right=0,label=$\scriptstyle l$,l.d=2.5,label.side=right}{v2t,v1}
\else\fi
\ifKV@FDinline@altmomentum
\fmf{electron,tension=0,right=0,label=$\scriptstyle l$,l.d=2.5,label.side=left}{v2b,v1}
\else\fi
% top double cut
\ifKV@FDinline@topdoublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2t}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v2b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,left=0,tension=0}{v1,v2t}
% \fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=left,right=0,tension=0}{v2t,v2b}
\fmfposition
 \fmfcmd{pair vert; vert = vloc(__v1);}
 % labels
 \fmfiv{label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.a=-5,l.d=30}{vert}
\else\fi
\else\fi
% bottom double cut
\ifKV@FDinline@botdoublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2b}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v2b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=right,left=0,tension=0}{v1,v2b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,right=0,tension=0}{v2t,v2b}
\else\fi
\else\fi
% double cut
\ifKV@FDinline@doublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2t}
\fmf{phantom_smallcut,right=0,tension=0}{v1,v2b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,left=0,tension=0}{v1,v2t}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=right,right=0,tension=0}{v1,v2b}
\else\fi
\else\fi
\else\fi
% TRIANGLETHREEBOT
\ifKV@FDinline@trianglethreebot
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% internal lines right
\fmf{plain,tension=1.5}{v2t,vp1}
\fmf{plain,tension=0}{v2b,vp2}
\fmf{plain,tension=1.5}{v2b,vp3}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,label.side=left,l.d=2.5}{v2b,v1}
\else\fi
\ifKV@FDinline@altmomentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,label.side=right,l.d=2.5}{v2t,v1}
\else\fi
% top double cut
\ifKV@FDinline@topdoublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2t}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v2b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,left=0,tension=0}{v1,v2t}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=left,right=0,tension=0}{v2t,v2b}
\else\fi
\else\fi
% bottom double cut
\ifKV@FDinline@botdoublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2b}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v2b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=right,left=0,tension=0}{v1,v2b}
% \fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,right=0,tension=0}{v2t,v2b}
\fmfposition
 \fmfcmd{pair vert; vert = vloc(__v1);}
 % labels
 \fmfiv{label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.a=5,l.d=30}{vert}
\else\fi
\else\fi
% double cut
\ifKV@FDinline@doublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2t}
\fmf{phantom_smallcut,right=0,tension=0}{v1,v2b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,left=0,tension=0}{v1,v2t}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=right,right=0,tension=0}{v1,v2b}
\else\fi
\else\fi
\else\fi
% DOUBLETRIANGLETHREE
\ifKV@FDinline@doubletrianglethree
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=6}{vq,v1}
% internal lines middle
\fmf{plain,left=0.0}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2m}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2m}
\fmf{plain,tension=0}{v2m,v2b}
% internal lines right
\fmf{plain,tension=2}{v2t,vp1}
\fmf{plain,tension=2}{v2m,vp2}
\fmf{plain,tension=2}{v2b,vp3}
% derivative momenta
\ifKV@FDinline@dermomenta
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,l.s=right,l.d=2.5}{v2t,v1}
\fmf{electron,tension=0,left=0,label=$\scriptstyle k$,l.s=left,l.d=2.5}{v2b,v1}
\else\fi
\else\fi
% BUBBLETRIANGLETHREE
\ifKV@FDinline@bubbletrianglethree
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=6}{vq,v1}
% internal lines middle
\fmf{phantom,left=0.0}{v1,v2t}
\fmf{plain,left=0.7,tension=0}{v1,v2m}
\fmf{plain,right=0.0}{v1,v2m}
\fmf{plain,right=0.0}{v1,v2b}
% \fmf{plain,tension=0}{v2t,v2m}
\fmf{plain,tension=0}{v2m,v2b}
% internal lines right
\fmf{phantom,tension=2}{v2t,vp1}
\fmf{plain,tension=0}{v2m,vp1}
\fmf{plain,tension=2}{v2m,vp2}
\fmf{plain,tension=2}{v2b,vp3}
\else\fi
% TRIANGLEBUBBLETHREE
\ifKV@FDinline@trianglebubblethree
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=6}{vq,v1}
% internal lines middle
\fmf{phantom,left=0.0}{v1,v2b}
\fmf{plain,right=0.7,tension=0}{v1,v2m}
\fmf{plain,right=0.0}{v1,v2m}
\fmf{plain,right=0.0}{v1,v2t}
% \fmf{plain,tension=0}{v2t,v2m}
\fmf{plain,tension=0}{v2m,v2t}
% internal lines right
\fmf{phantom,tension=2}{v2b,vp3}
\fmf{plain,tension=0}{v2m,vp3}
\fmf{plain,tension=2}{v2m,vp2}
\fmf{plain,tension=2}{v2t,vp1}
\else\fi
% DOUBLETRIANGLETWO
\ifKV@FDinline@doubletriangletwo
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=6}{vq,v1}
% internal lines middle
\fmf{plain,left=0.0}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2m}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2m}
\fmf{plain,tension=0}{v2m,v2b}
% internal lines right
\ifKV@FDinline@masstop
\fmf{double,tension=2}{v2t,vp1}
\else
\fmf{plain,tension=2}{v2t,vp1}
\fi
\ifKV@FDinline@massbottom
\fmf{double,tension=2}{v2b,vp3}
\else
\fmf{plain,tension=2}{v2b,vp3}
\fi
\fmf{phantom,tension=2}{v2m,vp2}
% derivative momenta
\ifKV@FDinline@dermomenta
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,l.s=right,l.d=2.5}{v2t,v1}
\fmf{electron,tension=0,left=0,label=$\scriptstyle k$,l.s=left,l.d=2.5}{v2b,v1}
\else\fi
\else\fi
% ITWO
\ifKV@FDinline@itwo
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0,right=0.5}{v2t,v2b}
\fmf{plain,tension=0,left=0.5}{v2t,v2b}
% internal lines right
\fmf{plain,tension=1.5}{v2t,vp1}
\fmf{plain,tension=1.5}{v2b,vp2}
\else\fi
% RAINBOW
\ifKV@FDinline@rainbow
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.0,tension=0.8,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0,tension=0.8}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,label.side=right,l.d=2.5}{v2t,v1}
\else\fi
% momentum arrow
\ifKV@FDinline@momentumarrow
\fmf{electron,tension=0,left=0}{v2t,v1}
\else\fi
% internal lines middle right
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v2t,v3t}
\fmf{plain,right=0.0}{v2b,v3b}
\fmf{plain,tension=0}{v3t,v3b}
% internal lines right
\fmf{plain,tension=1.5}{v3t,vp1}
\fmf{plain,tension=1.5}{v3b,vp2}
% triple cut
\ifKV@FDinline@triplecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2t}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v2b}
\fmf{phantom_smallcut,right=0,tension=0}{v2b,v3b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,left=0,tension=0}{v1,v2t}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=left,right=0,tension=0}{v2t,v2b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,l.d=8,label.side=right,right=0,tension=0}{v2b,v3b}
\else\fi
\else\fi
% alternative triple cut
\ifKV@FDinline@alttriplecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2b}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v2b}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v3t}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,l.d=8,label.side=right,left=0,tension=0}{v1,v2b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=left,right=0,tension=0}{v2t,v2b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,right=0,tension=0}{v2t,v3t}
\else\fi
\else\fi
% quadruple cut
\ifKV@FDinline@quadruplecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2t}
\fmf{phantom_smallcut,right=0,tension=0}{v1,v2b}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v3t}
\fmf{phantom_smallcut,right=0,tension=0}{v2b,v3b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_4}$,l.d=12,label.side=left,left=0,tension=0}{v1,v2t}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,l.d=12,label.side=right,right=0,tension=0}{v1,v2b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=12,label.side=right,right=0,tension=0}{v2b,v3b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=12,label.side=left,right=0,tension=0}{v2t,v3t}
\else\fi
\else\fi
% double cut
\ifKV@FDinline@doublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2t}
\fmf{phantom_smallcut,right=0,tension=0}{v1,v2b}
% \fmf{phantom_smallcut,right=0,tension=0}{v2t,v3t}
% \fmf{phantom_smallcut,right=0,tension=0}{v2b,v3b}
% cutlabels
\ifKV@FDinline@cutlabels
 \fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,left=0,tension=0}{v1,v2t}
 \fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=right,right=0,tension=0}{v1,v2b}
% \fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=12,label.side=right,right=0,tension=0}{v2b,v3b}
% \fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=12,label.side=left,right=0,tension=0}{v2t,v3t}
\else\fi
\else\fi
\else\fi
% FLIPPED RAINBOW
\ifKV@FDinline@fliprainbow
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{phantom,left=0.0,tension=0.8}{vq,v2t}
\fmf{phantom,right=0.0,tension=0.8}{vq,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% internal lines middle left
\fmf{phantom,left=0.0,tension=0.0001,tag=1}{v1,v3t}
\fmf{phantom,right=0.0,tension=0.0001}{v1,v3b}
\fmf{plain,left=0.0,tension=0.00005}{v1,v2t}
\fmf{plain,right=0.0,tension=0.00005}{v1,v2b}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,label.side=left,l.d=2.5}{v2t,v1}
\else\fi
% internal lines middle right
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v2t,v3t}
\fmf{plain,right=0.0}{v2b,v3b}
\fmf{plain,tension=0,tag=1}{v3t,v3b}
% internal lines right
\fmf{plain,tension=1.8}{v3t,vp1}
\fmf{plain,tension=1.8}{v3b,vp2}
% double line
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v3t)}
\fmfiset{p2}{vpath1(__v3t,__v3b)}
% \fmfi{double}{point 0*length(p1)/2 of p1 -- point length(p2)/2 of p2}
\fmfi{double}{point 0*length(p1)/2 of p1 -- 0.5*((point length(p2)/2 of p2)+(point 0*length(p1)/2 of p1))}
% triple cut
\ifKV@FDinline@triplecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2t}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v2b}
\fmf{phantom_smallcut,right=0,tension=0}{v2b,v3b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=13,label.side=right,left=0,tension=0}{v1,v2t}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=right,right=0,tension=0}{v2t,v2b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,l.d=8,label.side=right,right=0,tension=0}{v2b,v3b}
\else\fi
\else\fi
% alternative triple cut
\ifKV@FDinline@alttriplecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2b}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v2b}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v3t}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=13,label.side=left,left=0,tension=0}{v1,v2b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,l.d=8,label.side=right,right=0,tension=0}{v2t,v2b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=left,right=0,tension=0}{v2t,v3t}
\else\fi
\else\fi
% quadruple cut
\ifKV@FDinline@quadruplecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,v2t}
\fmf{phantom_smallcut,right=0,tension=0}{v1,v2b}
\fmf{phantom_smallcut,right=0,tension=0}{v2t,v3t}
\fmf{phantom_smallcut,right=0,tension=0}{v2b,v3b}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=12,label.side=left,left=0,tension=0}{v1,v2t}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=12,label.side=right,right=0,tension=0}{v1,v2b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_4}$,l.d=12,label.side=right,right=0,tension=0}{v2b,v3b}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,l.d=12,label.side=left,right=0,tension=0}{v2t,v3t}
\else\fi
\else\fi
\else\fi
% BOXTRIANGLE
\fmfstraight
\ifKV@FDinline@boxtriangle
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=6}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.0}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,right=0.0}{v1,v2m}
\fmf{plain,tension=0}{v2m,v2b}
% internal lines middle right
\fmf{plain,left=0.0,tension=2}{v2t,v3t}
\fmf{plain,right=0.0,tension=2}{v2b,v3b}
\fmf{plain,right=0.0,tension=2}{v2m,v3m}
\fmf{plain,tension=0}{v3t,v3m}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,l.d=2}{v2m,v3m}
\else\fi
% derivative momenta
\ifKV@FDinline@dermomenta
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,l.s=right,l.d=2.5}{v3t,v1}
\fmf{electron,tension=0,left=0,label=$\scriptstyle k$,l.s=left,l.d=2.5}{v2b,v1}
\else\fi
% internal lines right
\fmf{plain,tension=2}{v3t,vp1}
\fmf{plain,tension=2}{v3b,vp3}
\fmf{plain,tension=2}{v3m,vp2}
\else\fi
% TRIANGLEBOX
\fmfstraight
\ifKV@FDinline@trianglebox
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=6}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.0}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,right=0.0}{v1,v2m}
\fmf{plain,tension=0}{v2t,v2m}
% internal lines middle right
\fmf{plain,left=0.0,tension=2}{v2t,v3t}
\fmf{plain,right=0.0,tension=2}{v2b,v3b}
\fmf{plain,right=0.0,tension=2}{v2m,v3m}
\fmf{plain,tension=0}{v3m,v3b}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,l.s=left,l.d=2}{v2m,v3m}
\else\fi
% derivative momenta
\ifKV@FDinline@dermomenta
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,l.s=right,l.d=2.5}{v2t,v1}
\fmf{electron,tension=0,left=0,label=$\scriptstyle k$,l.s=left,l.d=2.5}{v3b,v1}
\else\fi
% internal lines right
\fmf{plain,tension=2}{v3t,vp1}
\fmf{plain,tension=2}{v3b,vp3}
\fmf{plain,tension=2}{v3m,vp2}
\else\fi
% WEDGETOP
\ifKV@FDinline@wedgetop
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% internal lines middle right
\fmf{plain,right=0.0}{v2b,v3b}
\fmf{plain,tension=0}{v2t,v3b}
% internal lines right
\fmf{plain,tension=1.5}{v2t,vp1}
\fmf{plain,tension=1.5}{v3b,vp2}
\else\fi
% WEDGESTARTOP
\ifKV@FDinline@wedgestartop
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
% internal lines middle right
\fmf{plain,right=0.0}{v2b,v3b}
% internal lines right
\fmf{plain,tension=1.5}{v2t,vp1}
\fmf{plain,tension=1.5}{v3b,vp2}
% middle
\fmffreeze
\fmf{plain,tension=1}{v2t,vm}
\fmf{plain,tension=0}{vm,v2b}
\fmf{plain,tension=1}{vm,v3b}
\else\fi
% WEDGEBOTTOM
\ifKV@FDinline@wedgebottom
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% internal lines middle right
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v2t,v3t}
\fmf{plain,tension=0}{v3t,v2b}
% internal lines right
\fmf{plain,tension=1.5}{v3t,vp1}
\fmf{plain,tension=1.5}{v2b,vp2}
\else\fi
% WEDGESTARBOTTOM
\ifKV@FDinline@wedgestarbottom
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
% internal lines middle right
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v2t,v3t}
% internal lines right
\fmf{plain,tension=1.5}{v3t,vp1}
\fmf{plain,tension=1.5}{v2b,vp2}
% middle
\fmffreeze
\fmf{plain,tension=1}{v2b,vm}
\fmf{plain,tension=0}{vm,v2t}
\fmf{plain,tension=1}{vm,v3t}
\else\fi
% RAINBOW NONPLANAR
\ifKV@FDinline@rainbownonplanar
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.0,tension=0.8,label=\FDinlinetoplabel}{v1,v2t}
\fmf{plain,right=0.0,tension=0.8}{v1,v2b}
\fmf{plain,tension=0,rubout}{v2t,v3b}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,l.d=2.5}{v2t,v1}
\else\fi
% internal lines middle right
\fmf{plain,left=0.0,label=\FDinlinetoplabel}{v2t,v3t}
\fmf{plain,right=0.0}{v2b,v3b}
\fmf{plain,tension=0}{v3t,v2b}
% internal lines right
\fmf{plain,tension=1.5}{v3t,vp1}
\fmf{plain,tension=1.5}{v3b,vp2}
\else\fi
% FLIPPED RAINBOW NONPLANAR
\ifKV@FDinline@fliprainbownonplanar
% outgoing
\fmfleft{vp1}
\fmfright{vp2}
\fmftop{vt}
\fmfbottom{vb}
% internal lines left
\fmf{plain,tension=5}{vp1,vl}
% internal lines middle
\fmf{phantom,tension=10}{vt,vta}
\fmf{plain,tension=1}{vta,v1}
\fmf{plain,tension=1}{vba,v1}
\fmf{phantom,tension=10}{vba,vb}
% internal lines middle left
\fmf{plain,tension=1}{vta,vl}
\fmf{plain,tension=1}{vba,vl}
% internal lines middle right
\fmf{plain,tension=1}{vta,vr}
\fmf{plain,tension=1}{vba,vr}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,l.d=2.5,label.side=right}{v1,vta}
\else\fi
% momentum arrow
\ifKV@FDinline@momentumarrow
\fmf{electron,tension=0,left=0}{vta,v1}
\else\fi
% internal lines right
\fmf{plain,tension=5}{vr,vp2}
% double line
\fmf{phantom,tension=0,tag=1}{vl,v1}
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__vl,__v1)}
\fmfi{double}{subpath (length(p1),0.6*length(p1)) of p1}
% triple cut
\ifKV@FDinline@triplecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,vta}
\fmf{phantom_smallcut,right=0,tension=0}{vr,vba}
\fmf{phantom_smallcut,right=0,tension=0}{vl,vba}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=12,label.side=right,left=0,tension=0}{v1,vta}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=12,label.side=left,right=0,tension=0}{vr,vba}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,l.d=12,label.side=right,right=0,tension=0}{vl,vba}
\else\fi
\else\fi
% alternative triple cut
\ifKV@FDinline@alttriplecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,vba}
\fmf{phantom_smallcut,right=0,tension=0}{vta,vl}
\fmf{phantom_smallcut,right=0,tension=0}{vta,vr}
% cutlabels
\ifKV@FDinline@cutlabels
 \fmfcmd{pair vert; vert = vloc(__v1);}
 % labels
%  \fmfiv{label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.a=+25,l.d=7}{vert}
 \fmfiv{label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.a=-25,l.d=7}{vert}
% \fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=left,left=0,tension=0}{v1,vba}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=right,right=0,tension=0}{vr,vta}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,l.d=8,label.side=left,right=0,tension=0}{vl,vta}
\else\fi
\else\fi
% quadruple cut
\ifKV@FDinline@quadruplecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,vta}
\fmf{phantom_smallcut,right=0,tension=0}{v1,vba}
\fmf{phantom_smallcut,right=0,tension=0}{vta,vr}
\fmf{phantom_smallcut,right=0,tension=0}{vba,vl}
% cutlabels
\ifKV@FDinline@cutlabels
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=12,label.side=left,left=0,tension=0}{v1,vta}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=12,label.side=left,right=0,tension=0}{v1,vba}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_4}$,l.d=12,label.side=left,right=0,tension=0}{vta,vr}
\fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,l.d=12,label.side=left,right=0,tension=0}{vba,vl}
\else\fi
\else\fi
% double cut
\ifKV@FDinline@doublecut
\fmf{phantom_smallcut,left=0,tension=0}{v1,vta}
\fmf{phantom_smallcut,right=0,tension=0}{v1,vba}
% \fmf{phantom_smallcut,right=0,tension=0}{vta,vr}
% \fmf{phantom_smallcut,right=0,tension=0}{vba,vl}
% cutlabels
\ifKV@FDinline@cutlabels
% \fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.d=8,label.side=right,left=0,tension=0}{v1,vta}
% \fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.d=8,label.side=left,right=0,tension=0}{v1,vba}
 \fmfcmd{pair vert; vert = vloc(__v1);}
 % labels
 \fmfiv{label=$\scriptstyle \textcolor{labelcolor}{l_1}$,l.a=+25,l.d=7}{vert}
 \fmfiv{label=$\scriptstyle \textcolor{labelcolor}{l_2}$,l.a=-25,l.d=7}{vert}
% \fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_4}$,l.d=12,label.side=left,right=0,tension=0}{vta,vr}
% \fmf{phantom,label=$\scriptstyle \textcolor{labelcolor}{l_3}$,l.d=12,label.side=left,right=0,tension=0}{vba,vl}
\else\fi
\else\fi
\else\fi
% TRIANGLEFISHTOP
\ifKV@FDinline@trianglefishtop
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0,tag=1,tension=0.5}{v1,v2t}
\fmf{plain,left=0,tag=2,tension=0.5}{v2b,v1}
% internal lines right
\fmf{plain,tension=2}{v2t,vp1}
\fmf{plain,tension=2}{v2b,vp2}
\fmf{plain,tension=0}{v2b,v2t}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2t)}
\fmfiset{p2}{vpath2(__v2b,__v1)}
\fmfi{plain}{(point 2length(p1)/3 of p1){dir -90}..{dir 180}(point length(p2) of p2)}
% derivative momenta
\ifKV@FDinline@dermomenta
\fmfi{electron,tension=0,left=0,label=$\scriptstyle l$,l.s=right,l.d=2.5}{(point 2length(p1)/3 of p1)..(point length(p2) of p2)}
\fmf{electron,tension=0,left=0,label=$\scriptstyle k$,l.s=left,l.d=2.5}{v2b,v1}
\else\fi
\else\fi
% TRIANGLEFISHBOTTOMBACK
\ifKV@FDinline@trianglefishbottomback
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0,tag=1,tension=0.5}{v1,v2t}
\fmf{plain,left=0,tag=2,tension=0.5}{v2b,v1}
% internal lines right
\fmf{plain,tension=2}{v2t,vp1}
\fmf{plain,tension=2}{v2b,vp2}
\fmf{plain,tension=0}{v2b,v2t}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2t)}
\fmfiset{p2}{vpath2(__v2b,__v1)}
\fmfi{plain}{(point 2length(p2)/3 of p2){dir 30}..{dir -70}(point 0length(p2) of p2)}
\else\fi
% TRIANGLEFISHTOPBACK
\ifKV@FDinline@trianglefishtopback
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0,tag=1,tension=0.5}{v1,v2t}
\fmf{plain,left=0,tag=2,tension=0.5}{v2b,v1}
% internal lines right
\fmf{plain,tension=2}{v2t,vp1}
\fmf{plain,tension=2}{v2b,vp2}
\fmf{plain,tension=0}{v2b,v2t}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2t)}
\fmfiset{p2}{vpath2(__v2b,__v1)}
\fmfi{plain}{(point 1length(p1)/3 of p1){dir -30}..{dir 70}(point length(p1) of p1)}
\else\fi
% TRIANGLEFISHBOTTOM
\ifKV@FDinline@trianglefishbottom
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0,tag=1,tension=0.5}{v1,v2t}
\fmf{plain,left=0,tag=2,tension=0.5}{v2b,v1}
% internal lines right
\fmf{plain,tension=2}{v2t,vp1}
\fmf{plain,tension=2}{v2b,vp2}
\fmf{plain,tension=0}{v2b,v2t}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2t)}
\fmfiset{p2}{vpath2(__v2b,__v1)}
\fmfi{plain}{(point 1length(p2)/3 of p2){dir 90}..{dir 180}(point length(p2) of p2)}
% derivative momenta
\ifKV@FDinline@dermomenta
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,l.s=right,l.d=2.5}{v2t,v1}
\fmfi{electron,tension=0,left=0,label=$\scriptstyle k$,l.s=left,l.d=2.5}{(point 1length(p2)/3 of p2)..(point length(p2) of p2)}
\else\fi
\else\fi
% TRIANGLESUBBUBBLEBOTTOM
\ifKV@FDinline@trianglesubbubblebottom
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0,tag=1,tension=0.5}{v1,v2t}
\fmf{plain,left=0,tag=2,tension=0.5}{v2b,v1}
% internal lines right
\ifKV@FDinline@masstop
\fmf{double,tension=2}{v2t,vp1}
\else
\fmf{plain,tension=2}{v2t,vp1}
\fi
\ifKV@FDinline@massbottom
\fmf{double,tension=2}{v2b,vp2}
\else
\fmf{plain,tension=2}{v2b,vp2}
\fi
\fmf{plain,tension=0}{v2b,v2t}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2t)}
\fmfiset{p2}{vpath2(__v2b,__v1)}
\fmfi{plain}{(point length(p2) of p2){dir 0}..{dir -70}(point 0length(p2) of p2)}
% derivative momenta
\ifKV@FDinline@dermomenta
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,l.s=right,l.d=2.5}{v2t,v1}
\fmf{electron,tension=0,left=0,label=$\scriptstyle k$,l.s=left,l.d=2.5}{v2b,v1}
\else\fi
\else\fi
% TRIANGLESUBBUBBLETOP
\ifKV@FDinline@trianglesubbubbletop
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{double,tension=4}{vq,v1}
% internal lines middle
\fmf{plain,left=0,tag=1,tension=0.5}{v1,v2t}
\fmf{plain,left=0,tag=2,tension=0.5}{v2b,v1}
% internal lines right
\ifKV@FDinline@masstop
\fmf{double,tension=2}{v2t,vp1}
\else
\fmf{plain,tension=2}{v2t,vp1}
\fi
\ifKV@FDinline@massbottom
\fmf{double,tension=2}{v2b,vp2}
\else
\fmf{plain,tension=2}{v2b,vp2}
\fi
\fmf{plain,tension=0}{v2b,v2t}
% internal lines middle vertical
\fmfposition
\fmfipath{p[]}
\fmfiset{p1}{vpath1(__v1,__v2t)}
\fmfiset{p2}{vpath2(__v2b,__v1)}
\fmfi{plain}{(point 0length(p1) of p1){dir 0}..{dir 70}(point length(p1) of p1)}
% derivative momenta
\ifKV@FDinline@dermomenta
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,l.s=right,l.d=2.5}{v2t,v1}
\fmf{electron,tension=0,left=0,label=$\scriptstyle k$,l.s=left,l.d=2.5}{v2b,v1}
\else\fi
\else\fi
% BOXBUBBLE
\fmfstraight
\ifKV@FDinline@boxbubble
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=6}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.0}{v1,v2t}
\fmf{plain,right=0.0,tension=1}{v1,v2m}
\fmf{phantom,right=0.0}{v1,v2b}
\fmf{plain,right=0.7,tension=0}{v1,v2m}
% internal lines middle right
\fmf{plain,left=0.0,tension=2}{v2t,v3t}
\fmf{plain,right=0.0,tension=2}{v2m,v3m}
\fmf{phantom,right=0.0,tension=2}{v2b,v3b}
\fmf{plain,tension=0}{v3t,v3m}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,l.d=2.5}{v2m,v3m}
\else\fi
% internal lines right
\fmf{plain,tension=2}{v3t,vp1}
\fmf{plain,tension=0}{v2m,vp3}
\fmf{phantom,tension=2}{v3b,vp3}
\fmf{plain,tension=2}{v3m,vp2}
\else\fi
% BUBBLEBOX
\fmfstraight
\ifKV@FDinline@bubblebox
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=6}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.7,tension=0}{v1,v2m}
\fmf{phantom,left=0.0}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,right=0.0,tension=1}{v1,v2m}
% internal lines middle right
\fmf{phantom,left=0.0,tension=2}{v2t,v3t}
\fmf{plain,right=0.0,tension=2}{v2b,v3b}
\fmf{plain,right=0.0,tension=2}{v2m,v3m}
\fmf{plain,tension=0}{v3m,v3b}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,l.d=2.5}{v2m,v3m}
\else\fi
% internal lines right
\fmf{plain,tension=0}{v2m,vp1}
\fmf{phantom,tension=2}{v3t,vp1}
\fmf{plain,tension=2}{v3b,vp3}
\fmf{plain,tension=2}{v3m,vp2}
\else\fi
% SHIFTEDTRIANGLETRIANGLE
\fmfstraight
\ifKV@FDinline@shiftedtriangletriangle
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=6}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.7,tension=0}{v1,v3m}
\fmf{phantom,left=0.0}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,right=0.0,tension=1}{v1,v2m}
% internal lines middle right
\fmf{phantom,left=0.0,tension=2}{v2t,v3t}
\fmf{plain,right=0.0,tension=2}{v2b,v3b}
\fmf{plain,right=0.0,tension=2}{v2m,v3m}
\fmf{plain,tension=0}{v2m,v2b}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,l.d=2}{v2m,v3m}
\else\fi
% internal lines right
\fmf{plain,tension=0}{v3m,vp1}
\fmf{phantom,tension=2}{v3t,vp1}
\fmf{plain,tension=2}{v3b,vp3}
\fmf{plain,tension=2}{v3m,vp2}
\else\fi
% SHIFTEDTRIANGLEBUBBLE
\fmfstraight
\ifKV@FDinline@shiftedtrianglebubble
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=6}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.7,tension=0}{v1,v3m}
\fmf{plain,right=0.7,tension=0}{v1,v2m}
\fmf{phantom,left=0.0}{v1,v2t}
\fmf{phantom,right=0.0}{v1,v2b}
\fmf{plain,right=0.0,tension=1}{v1,v2m}
% internal lines middle right
\fmf{phantom,left=0.0,tension=2}{v2t,v3t}
\fmf{phantom,right=0.0,tension=2}{v2b,v3b}
\fmf{plain,right=0.0,tension=2}{v2m,v3m}
% \fmf{plain,tension=0}{v2m,v2b}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,l.d=2.5}{v2m,v3m}
\else\fi
% internal lines right
\fmf{plain,tension=0}{v3m,vp1}
\fmf{phantom,tension=2}{v3t,vp1}
\fmf{plain,tension=0}{v2m,vp3}
\fmf{phantom,tension=2}{v3b,vp3}
\fmf{plain,tension=2}{v3m,vp2}
\else\fi
% BUBBLESHIFTEDTRIANGLE
\fmfstraight
\ifKV@FDinline@bubbleshiftedtriangle
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=6}{vq,v1}
% internal lines middle left
\fmf{plain,left=0.7,tension=0}{v1,v2m}
\fmf{plain,right=0.7,tension=0}{v1,v3m}
\fmf{phantom,left=0.0}{v1,v2t}
\fmf{phantom,right=0.0}{v1,v2b}
\fmf{plain,right=0.0,tension=1}{v1,v2m}
% internal lines middle right
\fmf{phantom,left=0.0,tension=2}{v2t,v3t}
\fmf{phantom,right=0.0,tension=2}{v2b,v3b}
\fmf{plain,right=0.0,tension=2}{v2m,v3m}
% \fmf{plain,tension=0}{v2m,v2b}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,l.d=2.5}{v2m,v3m}
\else\fi
% internal lines right
\fmf{plain,tension=0}{v2m,vp1}
\fmf{phantom,tension=2}{v3t,vp1}
\fmf{plain,tension=0}{v3m,vp3}
\fmf{phantom,tension=2}{v3b,vp3}
\fmf{plain,tension=2}{v3m,vp2}
\else\fi
% TRIANGLESHIFTEDTRIANGLE
\fmfstraight
\ifKV@FDinline@triangleshiftedtriangle
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{double,tension=6}{vq,v1}
% internal lines middle left
\fmf{plain,right=0.7,tension=0}{v1,v3m}
\fmf{phantom,left=0.0}{v1,v2b}
\fmf{plain,right=0.0}{v1,v2t}
\fmf{plain,right=0.0,tension=1}{v1,v2m}
% internal lines middle right
\fmf{phantom,left=0.0,tension=2}{v2b,v3b}
\fmf{plain,right=0.0,tension=2}{v2t,v3t}
\fmf{plain,right=0.0,tension=2}{v2m,v3m}
\fmf{plain,tension=0}{v2m,v2t}
% momentum
\ifKV@FDinline@momentum
\fmf{electron,tension=0,left=0,label=$\scriptstyle l$,l.d=2,l.s=left}{v2m,v3m}
\else\fi
% internal lines right
\fmf{plain,tension=0}{v3m,vp3}
\fmf{plain,tension=2}{v3t,vp1}
\fmf{phantom,tension=2}{v3b,vp3}
\fmf{plain,tension=2}{v3m,vp2}
\else\fi
% LABELS
%
% THREE LABELS  
 \ifKV@FDinline@threelabels
 %%% Workaround for MetaPost 1.504 bug 
 \fmfcmd{pair vertpone, vertptwo, vertpthree; vertpone = vloc(__vp1); vertptwo = vloc(__vp2); vertpthree = vloc(__vp3);}
 % labels
 \fmfiv{label=$\scriptstyle \FDinlinelabelone$,l.a=0,l.d=4}{vertpone}
 \fmfiv{label=$\scriptstyle \FDinlinelabeltwo$,l.a=0,l.d=4}{vertptwo}
 \ifKV@FDinline@splitlabels
 \fmfiv{label=$\scriptstyle \FDinlinelabelthree$,l.a=180,l.d=4}{vertpthree}
 \else
 \fmfiv{label=$\scriptstyle \FDinlinelabelthree$,l.a=0,l.d=4}{vertpthree}
 \fi
 \else\fi
%
% TWO LABELS  
 \ifKV@FDinline@twolabels
 %%% Workaround for MetaPost 1.504 bug 
 \fmfcmd{pair vertpone, vertptwo, vertpthree; vertpone = vloc(__vp1); vertptwo = vloc(__vp2);}
 % labels
 \ifKV@FDinline@splitlabels
 \fmfiv{label=$\scriptstyle \FDinlinelabelone$,l.a=180,l.d=4}{vertpone}
 \fmfiv{label=$\scriptstyle \FDinlinelabeltwo$,l.a=0,l.d=4}{vertptwo}
 \else
 \fmfiv{label=$\scriptstyle \FDinlinelabelone$,l.a=0,l.d=4}{vertpone}
 \fmfiv{label=$\scriptstyle \FDinlinelabeltwo$,l.a=0,l.d=4}{vertptwo}
 \fi
 \else\fi
% \end{fmfshrink}
\end{fmfchar*}%
% Set back to curved galeries
 \fmfcurved
}}}%
%%% Distances for labels
% TWO LABELS  
 \ifKV@FDinline@twolabels
 \ifKV@FDinline@splitlabels
\ensuremath{\phantom{{\scriptstyle \FDinlinelabeltwo}}}
\else
\ensuremath{\phantom{\frac{\scriptstyle \FDinlinelabelone}{\scriptstyle \FDinlinelabeltwo}}}
\fi\else\fi
% THREE LABELS  
 \ifKV@FDinline@threelabels
 \ifKV@FDinline@splitlabels
\ensuremath{\phantom{\frac{\scriptstyle \FDinlinelabelone}{\scriptstyle \FDinlinelabeltwo}}}
\else
\ensuremath{\phantom{\frac{\scriptstyle \FDinlinelabelone}{\frac{\scriptstyle \FDinlinelabelone}{\scriptstyle \FDinlinelabelthree}}}}
 \fi\else\fi
}


%% in-line diagrams
% xkeyval definitions
\define@boolkey{FDdimred}{zigzagbubble}[true]{}
\define@boolkey{FDdimred}{scalarbubble}[true]{}
\define@boolkey{FDdimred}{gluonbubble}[true]{}
\define@boolkey{FDdimred}{zigzagfermion}[true]{}
\define@boolkey{FDdimred}{scalarfermion}[true]{}
\define@boolkey{FDdimred}{gluonfermion}[true]{}
\define@boolkey{FDdimred}{bubble}[true]{}
\define@boolkey{FDdimred}{triangle}[true]{}
\define@boolkey{FDdimred}{cut}[true]{}
\define@key{FDdimred}{toplabel}%
{\def\FDdimredtoplabel{#1}}%
\define@key{FDdimred}{topleglabel}%
{\def\FDdimredtopleglabel{#1}}%
\define@key{FDdimred}{bottomleglabel}%
{\def\FDdimredbottomleglabel{#1}}%
\presetkeys{FDdimred}{%
zigzagbubble=false,%
scalarbubble=false,%
gluonbubble=false,%
zigzagfermion=false,%
scalarfermion=false,%
gluonfermion=false,%
bubble=false,%
triangle=false,%
cut=false,%
toplabel=$\phantom{0}$,%
topleglabel=$\phantom{0}$,%
bottomleglabel=$\phantom{0}$%
}{}
% Makro / FeynMP definitions
\newcommand*\FDdimred[1][]{%
 \setkeys{FDdimred}{#1}%
% 
\settoheight{\eqoff}{$\times$}%
\setlength{\eqoff}{0.5\eqoff}%
\addtolength{\eqoff}{-8\unitlength}%
\raisebox{\eqoff}{%
\fmfframe(1,0)(1,0){%
\scalebox{1}{%
\begin{fmfchar*}(30,16)%
\fmfcmd{%
dash_len := 1.6mm; 
}%
\begin{fmfshrink}{0.5}
% cut
\ifKV@FDdimred@cut
\fmftop{vtop}
\fmfbottom{vbot}
\fmf{dashes}{vtop,vbot}
\else\fi
% SCALARBUBBLE
\ifKV@FDdimred@scalarbubble
% outgoing
\fmfleft{vq1,vq2}
\fmfright{vp2,vp1}
% internal lines left
\fmf{plain,tension=1}{vq1,v1}
\fmf{plain,tension=1}{vq2,v1}
% internal lines middle
\fmf{plain,left=0.7,label=\FDdimredtoplabel}{v1,v2}
\fmf{plain,right=0.7}{v1,v2}
% internal lines right
\fmf{plain,tension=1}{v2,vp1}
\fmf{plain,tension=1}{v2,vp2}
% labels
\fmfv{label=\FDdimredtopleglabel,l.a=0}{vp1}
\fmfv{label=\FDdimredbottomleglabel,l.a=0}{vp2}
\else\fi
% GLUONBUBBLE
\ifKV@FDdimred@gluonbubble
% outgoing
\fmfleft{vq1,vq2}
\fmfright{vp2,vp1}
% internal lines left
\fmf{plain,tension=1}{vq1,v1}
\fmf{plain,tension=1}{vq2,v1}
% internal lines middle
\fmf{wiggly,left=0.7,label=\FDdimredtoplabel}{v1,v2}
\fmf{wiggly,right=0.7}{v1,v2}
% internal lines right
\fmf{plain,tension=1}{v2,vp1}
\fmf{plain,tension=1}{v2,vp2}
% labels
\fmfv{label=\FDdimredtopleglabel,l.a=0}{vp1}
\fmfv{label=\FDdimredbottomleglabel,l.a=0}{vp2}
\else\fi
% ZIGZAGBUBBLE
\ifKV@FDdimred@zigzagbubble
% outgoing
\fmfleft{vq1,vq2}
\fmfright{vp2,vp1}
% internal lines left
\fmf{plain,tension=1}{vq1,v1}
\fmf{plain,tension=1}{vq2,v1}
% internal lines middle
\fmf{zigzag,left=0.7,label=\FDdimredtoplabel}{v1,v2}
\fmf{zigzag,right=0.7}{v1,v2}
% internal lines right
\fmf{plain,tension=1}{v2,vp1}
\fmf{plain,tension=1}{v2,vp2}
% labels
\fmfv{label=\FDdimredtopleglabel,l.a=0}{vp1}
\fmfv{label=\FDdimredbottomleglabel,l.a=0}{vp2}
\else\fi
% BUBBLE
\ifKV@FDdimred@bubble
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{plain,tension=2}{vq,v1}
% internal lines middle
\fmf{plain,left=0.7,label=\FDdimredtoplabel}{v1,v2}
\fmf{plain,right=0.7}{v1,v2}
% internal lines right
\fmf{plain,tension=1.2}{v2,vp1}
\fmf{plain,tension=1.2}{v2,vp2}
% labels
\fmfv{label=\FDdimredtopleglabel,l.a=0}{vp1}
\fmfv{label=\FDdimredbottomleglabel,l.a=0}{vp2}
\else\fi
% TRIANGLE
\ifKV@FDdimred@triangle
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{plain,tension=2}{vq,v1}
% internal lines middle
\fmf{plain,left=0.0,label=\FDdimredtoplabel}{v1,v2t}
\fmf{plain,right=0.0}{v1,v2b}
\fmf{plain,tension=0}{v2t,v2b}
% internal lines right
\fmf{plain,tension=1.2}{v2t,vp1}
\fmf{plain,tension=1.2}{v2b,vp2}
% labels
\fmfv{label=\FDdimredtopleglabel,l.a=0}{vp1}
\fmfv{label=\FDdimredbottomleglabel,l.a=0}{vp2}
\else\fi
% ZIGZAGFERMION
\ifKV@FDdimred@zigzagfermion
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{zigzag,tension=2}{vq,v1}
% internal lines right
\fmf{dashes,tension=1}{v1,vp1}
\fmf{dashes,tension=1}{v1,vp2}
% labels
\fmfv{label=\FDdimredtopleglabel,l.a=0}{vp1}
\fmfv{label=\FDdimredbottomleglabel,l.a=0}{vp2}
\else\fi
% SCALARFERMION
\ifKV@FDdimred@scalarfermion
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{plain,tension=2}{vq,v1}
% internal lines right
\fmf{dashes,tension=1}{v1,vp1}
\fmf{dashes,tension=1}{v1,vp2}
% labels
\fmfv{label=\FDdimredtopleglabel,l.a=0}{vp1}
\fmfv{label=\FDdimredbottomleglabel,l.a=0}{vp2}
\else\fi
% GLUONFERMION
\ifKV@FDdimred@gluonfermion
% outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{photon,tension=2}{vq,v1}
% internal lines right
\fmf{dashes,tension=1}{v1,vp1}
\fmf{dashes,tension=1}{v1,vp2}
% labels
\fmfv{label=\FDdimredtopleglabel,l.a=0}{vp1}
\fmfv{label=\FDdimredbottomleglabel,l.a=0}{vp2}
\else\fi
\end{fmfshrink}
\end{fmfchar*}%
}}}%
}


%% flow diagrams
% xkeyval definitions
\define@boolkey{FDflow}{spacetime}[true]{}
\define@boolkey{FDflow}{flavour}[true]{}
\define@boolkey{FDflow}{black}[true]{}
\define@boolkey{FDflow}{blue}[true]{}
\define@boolkey{FDflow}{green}[true]{}
\define@boolkey{FDflow}{red}[true]{}
\define@boolkey{FDflow}{fermion}[true]{}
\define@boolkey{FDflow}{twopoint}[true]{}
\define@boolkey{FDflow}{cutleft}[true]{}
\define@boolkey{FDflow}{cutright}[true]{}
\define@boolkey{FDflow}{cutmiddle}[true]{}
% \define@key{FDdimred}{bottomleglabel}%
% {\def\FDdimredbottomleglabel{#1}}%
\presetkeys{FDflow}{%
flavour=false,%
spacetime=false,%
black=false,%
blue=false,%
green=false,%
red=false,%
fermion=false,%
twopoint=false,%
cutmiddle=false,%
cutright=false,%
cutleft=false,%
% bottomleglabel=$\phantom{0}$%
}{}
% Makro / FeynMP definitions
\newcommand*\FDflow[1][]{%
 \setkeys{FDflow}{#1}%
%
\fmfstraight
%
\settoheight{\eqoff}{$\times$}%
\setlength{\eqoff}{0.5\eqoff}%
\addtolength{\eqoff}{-10\unitlength}%
\raisebox{\eqoff}{%
\fmfframe(0,3)(4,3){%
\scalebox{1}{%
\begin{fmfchar*}(25,14)%
\fmfcmd{%
dash_len := 1.6mm; 
}%
\begin{fmfshrink}{1}
% FERMIONS
\ifKV@FDflow@fermion
% outgoing
\fmfleft{vq}
\fmfright{vp3,vp2,vp1}
% internal lines left
\fmf{dbl_plain,tension=10}{vq,v1}
% internal lines middle
\fmf{phantom,left=1.0}{v1,v2}
\fmf{phantom,right=1.0}{v1,v2}
% internal lines right
\fmf{phantom,tension=1.0}{v2,vp1}
\fmf{phantom,tension=1.0}{v2,vp3}
\fmffreeze
\fmfdraw
 % labels  
 %%% Workaround for MetaPost 1.504 bug 
 \fmfcmd{pair vertq, vertpone, vertptwo, vertpthree, vertone, verttwo; vertone = vloc(__v1); verttwo = vloc(__v2); vertq = vloc(__vq); vertpone = vloc(__vp1); vertptwo = vloc(__vp2); vertpthree = vloc(__vp3);}
 % lines
 \fmfi{plain}{(vertone){dir 60}..{dir -45}(verttwo+(-20/sqrt(2),20/sqrt(2)))}
 \fmfi{plain}{(vertone){dir -60}..{dir 45}(verttwo+(-20/sqrt(2),-20/sqrt(2)))}
 \fmfi{plain}{(vertpone){dir -170}..{dir -135}(verttwo+(20/sqrt(2),20/sqrt(2)))}
 \fmfi{plain}{(vertptwo){dir -180}..{dir 0}(verttwo+(20,0))}
 \fmfi{plain}{(vertpthree){dir 170}..{dir 135}(verttwo+(20/sqrt(2),-20/sqrt(2)))}
% TWO-POINT FUNCTION
 \else
 \ifKV@FDflow@twopoint
 % outgoing
\fmfleft{vq1}
\fmfright{vq2}
% internal lines left
\fmf{dbl_plain,tension=10}{vq1,v1}
% internal lines middle
\fmf{phantom,left=1.0}{v1,v2}
\fmf{phantom,right=1.0}{v1,v2}
\fmf{phantom,left=1.0}{v2,v3}
\fmf{phantom,right=1.0}{v2,v3}
% internal lines right
\fmf{dbl_plain,tension=10}{v3,vq2}
\fmffreeze
\fmfdraw
 % labels  
 %%% Workaround for MetaPost 1.504 bug 
 \fmfcmd{pair vertqone,  vertqtwo, vertone, verttwo, vertthree; vertqone = vloc(__vq1); vertone = vloc(__v1);verttwo = vloc(__v2);vertthree = vloc(__v3); vertqtwo = vloc(__vq2); }
 % lines
 \fmfi{plain}{(vertone){dir 60}..{dir -45}(verttwo+(-20/sqrt(2),20/sqrt(2)))}
 \fmfi{plain}{(vertone){dir -60}..{dir 45}(verttwo+(-20/sqrt(2),-20/sqrt(2)))}
 \fmfi{plain}{(vertthree){dir 120}..{dir -135}(verttwo+(20/sqrt(2),20/sqrt(2)))}
 \fmfi{plain}{(vertthree){dir -120}..{dir 135}(verttwo+(20/sqrt(2),-20/sqrt(2)))}
 % SCALARS 
 \else
 % outgoing
\fmfleft{vq}
\fmfright{vp2,vp1}
% internal lines left
\fmf{dbl_plain,tension=10}{vq,v1}
% internal lines middle
\fmf{phantom,left=1.0}{v1,v2}
\fmf{phantom,right=1.0}{v1,v2}
% internal lines right
\fmf{phantom,tension=1.0}{v2,vp1}
\fmf{phantom,tension=1.0}{v2,vp2}
\fmffreeze
\fmfdraw
 % labels  
 %%% Workaround for MetaPost 1.504 bug 
 \fmfcmd{pair vertq, vertpone, vertptwo, vertone, verttwo; vertone = vloc(__v1); verttwo = vloc(__v2); vertq = vloc(__vq); vertpone = vloc(__vp1); vertptwo = vloc(__vp2);}
 % lines
 \fmfi{plain}{(vertone){dir 60}..{dir -45}(verttwo+(-20/sqrt(2),20/sqrt(2)))}
 \fmfi{plain}{(vertone){dir -60}..{dir 45}(verttwo+(-20/sqrt(2),-20/sqrt(2)))}
 \fmfi{plain}{(vertpone){dir -170}..{dir -135}(verttwo+(20/sqrt(2),20/sqrt(2)))}
 \fmfi{plain}{(vertptwo){dir 170}..{dir 135}(verttwo+(20/sqrt(2),-20/sqrt(2)))}
 \fi
 \fi
 % blobs
%  \fmfiv{label=$\cF^{(1)}_{\cO}$,l.d=0,l.a=0}{vertone}
 % labels external states
 \ifKV@FDflow@spacetime
 \ifKV@FDflow@twopoint
 \fmfiv{label=$\scriptstyle q$}{vertqone}
 \fmfiv{label=$\scriptstyle q$}{vertqtwo}
 \else
 \fmfiv{label=$\scriptstyle q$}{vertq}
 \fmfiv{l.a=0,label=$\scriptstyle p_1$}{vertpone}
 \fmfiv{l.a=0,label=$\scriptstyle p_2$}{vertptwo}
 \ifKV@FDflow@fermion
 \fmfiv{label=$\scriptstyle p_3$}{vertpthree}
\else\fi
\fi
\else\fi
%  \fmfiv{label=$\cdot$,l.d=20,l.a=-45}{vertone}
%  \fmfiv{label=$\cdot$,l.d=20,l.a=-60}{vertone}
%  \fmfiv{label=$\cdot$,l.d=20,l.a=-75}{vertone}
% 
\ifKV@FDflow@flavour
 \fmfiv{label=$\scriptstyle I$}{verttwo+(-16,14)}
 \fmfiv{label=$\scriptstyle J$}{verttwo+(-16,-14)}
 \ifKV@FDflow@fermion 
 \fmfiv{l.a=0,label=$\scriptstyle K$}{vertpone}
 \fmfiv{l.a=0,label=$\scriptstyle A$}{vertptwo}
 \fmfiv{l.a=0,label=$\scriptstyle B$}{vertpthree}
 \else
 \ifKV@FDflow@twopoint
 \fmfiv{label=$\scriptstyle K$}{verttwo+(+16,14)}
 \fmfiv{label=$\scriptstyle L$}{verttwo+(+16,-14)}
 \else
 \fmfiv{l.a=0,label=$\scriptstyle K$}{vertpone}
 \fmfiv{l.a=0,label=$\scriptstyle L$}{vertptwo}
 \fi
 \fi
\else\fi
% 
\ifKV@FDflow@black
 \fmfiv{decor.shape=circle,decor.filled=60,decor.size=40}{verttwo}
 \fmfiv{decor.shape=circle,decor.filled=0,decor.size=8}{verttwo+(7,7)}
 \fmfiv{decor.shape=circle,decor.filled=0,decor.size=8}{verttwo+(-7,7)}
 \fmfiv{decor.shape=circle,decor.filled=0,decor.size=8}{verttwo+(7,-7)}
 \fmfiv{decor.shape=circle,decor.filled=0,decor.size=8}{verttwo+(-7,-7)}
\else\fi
% 
\ifKV@FDflow@blue
  \fmfiv{decor.shape=circle,decor.filled=20,decor.size=40}{verttwo}
 \fmfdraw
 \ifKV@FDflow@fermion 
 \fmfi{plain,fore=blue}{(verttwo+(0,-8)){dir 90}..{dir 0}(verttwo+(20,0))}
 \else\fi
 \fmfi{plain,fore=blue}{(verttwo+(-20/sqrt(2),20/sqrt(2))){dir -45}..{dir 45}(verttwo+(20/sqrt(2),20/sqrt(2)))}
 \fmfi{plain,fore=blue}{(verttwo+(-20/sqrt(2),-20/sqrt(2))){dir 45}..{dir -45}(verttwo+(20/sqrt(2),-20/sqrt(2)))}
\else\fi
% 
\ifKV@FDflow@red
  \fmfiv{decor.shape=circle,decor.filled=20,decor.size=40}{verttwo}
 \fmfdraw
 \ifKV@FDflow@fermion 
 \fmfi{plain,fore=red}{(verttwo+(11,0)){dir 180}..{dir 0}(verttwo+(20,0))}
 \else\fi
 \fmfi{plain,fore=red}{(verttwo+(-20/sqrt(2),20/sqrt(2))){dir -45}..{dir -135}(verttwo+(-20/sqrt(2),-20/sqrt(2)))}
 \fmfi{plain,fore=red}{(verttwo+(20/sqrt(2),20/sqrt(2))){dir -135}..{dir -45}(verttwo+(20/sqrt(2),-20/sqrt(2)))}
\else\fi
% 
\ifKV@FDflow@green
  \fmfiv{decor.shape=circle,decor.filled=20,decor.size=40}{verttwo}
 \fmfdraw
 \ifKV@FDflow@fermion 
 \fmfi{plain,fore=green}{(verttwo+(10/sqrt(2),-10/sqrt(2))){dir +45}..{dir 0}(verttwo+(20,0))}
 \else\fi
 \fmfi{plain,fore=green}{(verttwo+(-20/sqrt(2),20/sqrt(2))){dir -45}..{dir -45}(verttwo+(20/sqrt(2),-20/sqrt(2)))}
 \fmfi{plain,fore=green}{(verttwo+(-20/sqrt(2),-20/sqrt(2))){dir 45}..{dir 45}(verttwo-(2/sqrt(2),2/sqrt(2)))}
 \fmfi{plain,fore=green}{(verttwo+(2/sqrt(2),2/sqrt(2))){dir 45}..{dir 45}(verttwo+(20/sqrt(2),20/sqrt(2)))}
\else\fi
\fmftop{vt}
\fmfbottom{vb}
\fmfposition
 %%% Workaround for MetaPost 1.504 bug 
 \fmfcmd{pair verttop, vertbot; verttop = vloc(__vt); vertbot = vloc(__vb); }
\ifKV@FDflow@cutmiddle
\fmfi{dashes}{(verttop+(0,8))--(vertbot+(0,-8))}
\else\fi
\ifKV@FDflow@cutleft
\fmfi{dashes}{(verttop+(-11,8))--(vertbot+(-11,-8))}
\else\fi
\ifKV@FDflow@cutright
\fmfi{dashes}{(verttop+(11,8))--(vertbot+(11,-8))}
\else\fi
\end{fmfshrink}
\end{fmfchar*}%
}}}%
}











\makeatother

\newcommand{\initialisepictures}{
\fmfcmd{%
thin := 1pt; % dimension of the lines
thick := 2thin;
arrow_len := 3mm;
arrow_ang := 15;
curly_len := 3mm;
dash_len :=0.5; % 'photon' lines
% dash_space := 4mm;
dot_len := 0.75mm; % 'photon' lines
wiggly_len := 2mm; % 'photon' lines
wiggly_slope := 60;
zigzag_len := 2mm;
zigzag_width := 2thick;
decor_size := 5mm;
dot_size := 2thick;
}
\fmfcmd{%
marksize=7mm;
%
def draw_cut(expr p,a) =
  begingroup
    save t,tip,dma,dmb; pair tip,dma,dmb;
    t=arctime a of p;
    tip =marksize*unitvector direction t of p;
    dma =marksize*unitvector direction t of p rotated -90;
    dmb =marksize*unitvector direction t of p rotated 90;
    linejoin:=beveled;
%     draw (-.5dma.. .5tip-- -.5dmb) shifted point t of p;
%     drawoptions(dashed evenly);
    drawoptions(dashed dashpattern(on 6bp off 12bp on 6bp));
    draw ((-.5dma.. -.5dmb) shifted point t of p);
    drawoptions();
  endgroup
enddef;
%
style_def phantom_cut expr p =
    save amid;
    amid=.5*arclength p;
    draw_cut(p, amid);
    draw p;
enddef;
}
\fmfcmd{%
smallmarksize=4mm;
%
def draw_smallcut(expr p,a) =
  begingroup
    save t,tip,dma,dmb; pair tip,dma,dmb;
    t=arctime a of p;
    tip =smallmarksize*unitvector direction t of p;
    dma =smallmarksize*unitvector direction t of p rotated -90;
    dmb =smallmarksize*unitvector direction t of p rotated 90;
    linejoin:=beveled;
%     draw (-.5dma.. .5tip-- -.5dmb) shifted point t of p;
%     drawoptions(dashed evenly);
    drawoptions(dashed dashpattern(on 2bp off 2bp on 2bp) withcolor red);
    draw ((-.5dma.. -.5dmb) shifted point t of p);
    drawoptions();
  endgroup
enddef;
%
style_def phantom_smallcut expr p =
    save amid;
    amid=.5*arclength p;
    draw_smallcut(p, amid);
    draw p;
enddef;
}
}
